A comparative study of split advection algorithms on Moment-of-Fluid (MOF) method for incompressible flow

The moment-of-fluid method (MOF) is known as an extension of the volume-of-fluid method with piecewise linear interface construction (VOF-PLIC). In this study, several directional splitting advection algorithms are extended from the VOF-PLIC method to the MOF method. Those methods, along with some existing directional splitting algorithms, are presented in detail, especially on the geometrical and non-geometrical nature of the advection algorithm. Besides, we also proposed a simple and efficient analytic form to calculate the volume and centroid of the intersection polyhedron in 3D. Several numerical tests, including both 2D and 3D tests, are carried out to investigate mass conservation and geometrical error. Numerical results suggest that the mixed EI and LE scheme (EILE2D) \citep{aulisa_geometrical_2003} has the best overall performance in 2D and Weymouth and Yue's scheme (WY) has the best overall performance in 3D.

==> figures.tex <==
%<*fig:sketchmof>
\begin{figure}[htbp]
    \centering
    \subfigure[]{\includegraphics[width=0.4\textwidth]{sketch_mof_centroid.pdf}}
    \subfigure[]{\includegraphics[width=0.5\textwidth]{sketch_mof_centroid_3d.png}}
    \caption{(a) 2D view and (b) 3D view of the MOF reconstruction. The red curve (surface) is the true interface and the blue line (surface) is the reconstructed interface by MOF. The centroid of the reconstruct interface (blue dot) is the optimized centroid that minimized the distance between the reconstructed centroid and the reference centroid (red dot) with same volume fraction.
    }
    \label{fig:sketchmof}
\end{figure}
%</fig:sketchmof>

%<*fig:cuts>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{cuts.pdf}
    \caption{Five configurations of the cutting polyhedron by a plane with the intersection of \smallskip
        (a) Triangle, \smallskip 
        (b)	Quadrilateral-1, \smallskip
        (c) Pentagon, \smallskip
        (d) hexagon, \smallskip
        (e) Quadrilateral-2.
    }
    \label{fig:cuts}
\end{figure}
%</fig:cuts>


%<*fig:EILEadvection>
\begin{figure}[htbp]
    \centering
    \subfigure[Eulerian implicit (EI) advection]{\includegraphics[width=0.6\textwidth]{eulerian_implicit.pdf}} \\
    \subfigure[Lagrangian explicit (LE) advection]{\includegraphics[width=0.6\textwidth]{lagrangian_explicit.pdf}}
    \caption{The Eulerian implicit scheme (EI) and Lagrangian Explicit (LE) scheme for advection of volume fraction and centroids from step $n$ to step $*$. The mapping procedure is indicated by the black dotted line and the gray dashed line indicates the flux region. The new volume fraction at time $*$ are determined by the summation of smaller pieces of polyhedrons. The new reconstruction interface and centroid are plotted with blue dashed line and blue cross, respectively.
    }
    \label{fig:EILE_advection}
\end{figure}
%</fig:EILEadvection>

%<*fig:eile2d>
\begin{figure}[htbp]
    \centering
    \subfigure[Mapping $\Pi_{xy}$]{\includegraphics[width=0.7\textwidth]{eiles.pdf}} \\
    \subfigure[Mapping $\Pi_{yx}$]{\includegraphics[width=0.7\textwidth]{eiles2.pdf}}
    \caption{Mapping from the departure region $\Omega_{depart}$ to the target region $\Omega_{target}$ during EILE2D advection. (a) Mapping $\Pi_{xy}$ starts with EI advection in $x$ direction then LE advection in $y$ direction. (b) Mapping $\Pi_{yx}$ starts with EI advection in $y$ direction and then LE advection in $x$ direction.
    }
    \label{fig:eile2d}
\end{figure}
%</fig:eile2d>

%<*fig:flood>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{flood.pdf}
    \caption{Flood algorithm.}
    \label{fig:flood}
\end{figure}
%</fig:flood>


%<*fig:2dzalesakinit>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{zalesak-sketch2d.pdf}
    \caption{Initial setup and parameters of 2D Zalesak's disk rotation test
    }
    \label{fig:2dzalesakinit}
\end{figure}
%</fig:2dzalesakinit>

%<*fig:2dzalesakcfls>
\begin{figure}[htbp]
    \centering
    \subfigure[CFL$=0.05$]
    {\includegraphics[width=0.5\textwidth]{zalesak2d-eg-cfl005.pdf}}
    \subfigure[CFL$=0.5$]
    {\includegraphics[width=0.5\textwidth]{zalesak2d-eg-cfl05.pdf}}
    \caption{Geometrical error of 2D Zalesak's disk rotation test with repeatedly halving grid resolution at (a) $\rm{CFL}=0.05$ and (b) $\rm{CFL}=0.5$. The correponding data is shown in Table \ref{tab:2dzalesakcfls}.
    }
    \label{fig:2dzalesakcfls}
\end{figure}
%</fig:2dzalesakcfls>

%<*fig:2dzalesakresos>
\begin{figure}[htbp]
    \centering
    {\includegraphics[width=0.5\textwidth]{zalesak2d-eg-n64.pdf}}
    \caption{Geometrical error of 2D Zalesak's disk rotation test with different CFL numbers. The corresponding data in shown in Table \ref{tab:2dzalesakresos}.}
    \label{fig:2dzalesakresos}
\end{figure}
%</fig:2dzalesakresos>


%<*fig:2dsvinit>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{sv-sketch2d.pdf}
    \caption{Initial setup and parameters of 2D Rider-Kothe single vortex test.
    }
    \label{fig:2dsvinit}
\end{figure}
%</fig:2dsvinit>

%<*fig:2dsvcontour>
\begin{figure}[htbp]
    \centering
    {\includegraphics[width=1.0\textwidth]{sv2dcompare.pdf}}
    \caption{Material interface for 2D Rider-Kothe single vortex test represent by volume fraction $C=0.5$ with different CFL numbers on a $64 \times 64$ mesh.
    }
    \label{fig:2dsvcontour}
\end{figure}
%</fig:2dsvcontour>

%<*fig:2dsvcfls>
\begin{figure}[htbp]
    \centering
    \subfigure[$E_g$, CFL$=0.05$]
    {\includegraphics[width=0.5\textwidth]{sv2d-eg-cfl005.pdf}}
    \subfigure[$E_m$, CFL$=0.05$]
    {\includegraphics[width=0.5\textwidth]{sv2d-em-cfl005.pdf}} \\

    \subfigure[$E_g$, CFL$=1.0$]
    {\includegraphics[width=0.5\textwidth]{sv2d-eg-cfl10.pdf}}
    \subfigure[$E_m$, CFL$=1.0$]
    {\includegraphics[width=0.5\textwidth]{sv2d-em-cfl10.pdf}}
    \caption{(a) Geometrical error and (b) mass error of 2D Roder-Kothe singe vortex test with repeatedly halving grid resolution. The correponding data in shown in Table \ref{tab:2dsvcfls} and Table \ref{tab:2dsvcflsmass}.}
    \label{fig:2dsvcfls}
\end{figure}
%</fig:2dsvcfls>

%<*fig:2dsvresos>
\begin{figure}[htbp]
    \centering
    \subfigure[$E_g$, $N=64$]
    {\includegraphics[width=0.5\textwidth]{sv2d-eg-n64.pdf}}
    \subfigure[$E_m$, $N=64$]
    {\includegraphics[width=0.5\textwidth]{sv2d-em-n64.pdf}}
    \caption{Geometric error and mass error of 2D Roder-Kothe singe vortex test with repeatedly halving grid resolution with CFL numbers of 0.05 and 1.0. The correponding data in shown in Table \ref{tab:2dsvresos} and Table \ref{tab:2dsvresosmass}.}
    \label{fig:2dsvresos}
\end{figure}
%</fig:2dsvresos>

%<*fig:2drvinit>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{rv-sketch2d.pdf}
    \caption{Initial setup and parameters of 2D reversed vortex test
    }
    \label{fig:2drvinit}
\end{figure}
%</fig:2drvinit>

%<*fig:2drvcontour>
\begin{figure}[htbp]
    \centering
    {\includegraphics[width=1.0\textwidth]{rv2dcompare.pdf}}
    \caption{Material interface for 2D reversed vortex test represent by volume fraction $C=0.5$ with different CFL numbers on a $64 \times 64$ mesh.}
    \label{fig:2drvcontour}
\end{figure}
%</fig:2drvcontour>

%<*fig:2drvcfls>
\begin{figure}[htbp]
    \centering
    \subfigure[$E_g$, CFL$=0.05$]
    {\includegraphics[width=0.5\textwidth]{rv2d-eg-cfl005.pdf}}
    \subfigure[$E_m$, CFL$=0.05$]
    {\includegraphics[width=0.5\textwidth]{rv2d-em-cfl005.pdf}} \\

    \subfigure[$E_g$, CFL$=1.0$]
    {\includegraphics[width=0.5\textwidth]{rv2d-eg-cfl10.pdf}}
    \subfigure[$E_m$, CFL$=1.0$]
    {\includegraphics[width=0.5\textwidth]{rv2d-em-cfl10.pdf}}
    \caption{Geometric error and mass error of 2D reversed vortex test with different CFL numbers on a $64 \times 64$ mesh. The correponding data in shown in Table \ref{tab:2drvcfls} and Table \ref{tab:2drvcflsmass}.}
    \label{fig:2drvcfls}
\end{figure}
%</fig:2drvcfls>

%<*fig:2drvresos>
\begin{figure}[htbp]
    \centering
    \subfigure[$E_g$, $N=64$]
    {\includegraphics[width=0.5\textwidth]{rv2d-eg-n64.pdf}}
    \subfigure[$E_m$, $N=64$]
    {\includegraphics[width=0.5\textwidth]{rv2d-em-n64.pdf}}
    \caption{(a) Geometric error and (b) mass error of 2D reversed vortex test with repeatedly halving grid resolution. The correponding data in shown in Table \ref{tab:2drvresos} and Table \ref{tab:2drvresosmass}.}
    \label{fig:2drvresos}
\end{figure}
%</fig:2drvresos>


%<*fig:3dzalesakinit>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{zalesak-sketch3d.pdf}
    \caption{Initial setup and parameters of 3D Zalesak's rotation test.
    }
    \label{fig:3dzalesakinit}
\end{figure}
%</fig:3dzalesakinit>

%<*fig:3dzalesakcfls>
\begin{figure}[htbp]
    \centering
    {\includegraphics[width=0.5\textwidth]{zalesak3d-eg-cfl03.pdf}}
    \caption{Geometric error with the repeatedly halving  grid resolution under a CFL number of 0.03. The correponding data in shown in Table \ref{tab:3dzalesakcfls}.}
    \label{fig:3dzalesakcfls}
\end{figure}
%</fig:3dzalesakcfls>

%<*fig:3dzalesakresos>
\begin{figure}[htbp]
    \centering
    {\includegraphics[width=0.5\textwidth]{zalesak3d-eg-n64.pdf}}
    \caption{Geometric error with the change of CFL number on a $64 \times 64 \times 64$ mesh. The correponding data in shown in Table \ref{tab:3dzalesakresos}.}
    \label{fig:3dzalesakresos}
\end{figure}
%</fig:3dzalesakresos>

%<*fig:3dsvinit>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{sv-sketch3d.pdf}
    \caption{Initial setup and parameters of 3D single vortex test.
    }
    \label{fig:3dsvinit}
\end{figure}
%</fig:3dsvinit>

%<*fig:3dsvcfls>
\begin{figure}[htbp]
    \centering
    \subfigure[$E_g$, CFL$=0.05$]
    {\includegraphics[width=0.5\textwidth]{sv3d-eg-cfl05.pdf}}
    \subfigure[$E_m$, CFL$=0.05$]
    {\includegraphics[width=0.5\textwidth]{sv3d-em-cfl05.pdf}} \\

    \subfigure[$E_g$, CFL$=1.0$]
    {\includegraphics[width=0.5\textwidth]{sv3d-eg-cfl10.pdf}}
    \subfigure[$E_m$, CFL$=1.0$]
    {\includegraphics[width=0.5\textwidth]{sv3d-em-cfl10.pdf}}
    \caption{Geometric error and mass error of 3D reversed vortex test with repeated halving grid resolution under CFL number of 0.3 and 1.0. The correponding data in shown in Table \ref{tab:3dsvcfls} and Table \ref{tab:3dsvcflsmass}.}
    \label{fig:3dsvcfls}
\end{figure}
%</fig:3dsvcfls>

%<*fig:3dsvresos>
\begin{figure}[htbp]
    \centering
    \subfigure[$E_g$, $N=64$]
    {\includegraphics[width=0.5\textwidth]{sv3d-eg-n64.pdf}}
    \subfigure[$E_m$, $N=64$]
    {\includegraphics[width=0.5\textwidth]{sv3d-em-n64.pdf}}
    \caption{(a) Geometric error and (b) mass error of 3D reversed vortex test with the change of CFL number on a $32 \times 32 \times 64$ mesh. The correponding data in shown in Table \ref{tab:3dsvresos} and Table \ref{tab:3dsvresosmass}.}
    \label{fig:3dsvresos}
\end{figure}
%</fig:3dsvresos>

%<*fig:3drvinit>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{rv-sketch3d.pdf}
    \caption{Initial setup and parameters of 3D reversed vortex rotation test
    }
    \label{fig:3drvinit}
\end{figure}
%</fig:3drvinit>

%<*fig:3drvcfls>
\begin{figure}[htbp]
    \centering
    \subfigure[$E_g$, CFL$=0.3$]
    {\includegraphics[width=0.5\textwidth]{rv3d-eg-cfl03.pdf}}
    \subfigure[$E_m$, CFL$=0.3$]
    {\includegraphics[width=0.5\textwidth]{rv3d-em-cfl03.pdf}} \\

    \subfigure[$E_g$, CFL$=1.0$]
    {\includegraphics[width=0.5\textwidth]{rv3d-eg-cfl10.pdf}}
    \subfigure[$E_m$, CFL$=1.0$]
    {\includegraphics[width=0.5\textwidth]{rv3d-em-cfl10.pdf}}
    \caption{Geometric error and mass error of 3D reversed vortex test with repeated halving grid resolution under CFL number of 0.3 and 1.0. The correponding data in shown in Table \ref{tab:3drvcfls} and Table \ref{tab:3drvcflsmass}.}
    \label{fig:3drvcfls}
\end{figure}
%</fig:3drvcfls>

%<*fig:3drvresos>
\begin{figure}[htbp]
    \centering
    \subfigure[$E_g$, $N=64$]
    {\includegraphics[width=0.5\textwidth]{rv3d-eg-n64.pdf}}
    \subfigure[$E_m$, $N=64$]
    {\includegraphics[width=0.5\textwidth]{rv3d-em-n64.pdf}}
    \caption{(a) Geometric error and (b) mass error of 3D reversed vortex test with the change of CFL number on a $64 \times 64 \times 64$ mesh. The corresponding data in shown in Table \ref{tab:3drvresos} and Table \ref{tab:3drvresosmass}.}
    \label{fig:3drvresos}
\end{figure}
%</fig:3drvresos>


%<*fig:3dsviso1>
\begin{figure}[htbp]
    \centering
    {\includegraphics[width=0.15\textwidth]{sv-front-exact-2.png}}
    {\includegraphics[width=0.15\textwidth]{front-320-EI.png}}
    {\includegraphics[width=0.15\textwidth]{front-320-LE.png}}
    {\includegraphics[width=0.15\textwidth]{front-320-EILE3D.png}}
    {\includegraphics[width=0.15\textwidth]{front-320-EILE3DS.png}}
    {\includegraphics[width=0.15\textwidth]{front-320-EIEALE.png}}
    {\includegraphics[width=0.15\textwidth]{front-320-WY.png}} \\

    \subfigure[Exact]
    {\includegraphics[width=0.15\textwidth]{sv-top-exact-2.png}}
    \subfigure[EI]
    {\includegraphics[width=0.15\textwidth]{top-320-EI.png}}
    \subfigure[LE]
    {\includegraphics[width=0.15\textwidth]{top-320-LE.png}}
    \subfigure[EILE3D]
    {\includegraphics[width=0.15\textwidth]{top-320-EILE3D.png}}
    \subfigure[EILE3DS]
    {\includegraphics[width=0.15\textwidth]{top-320-EILE3DS.png}}
    \subfigure[EIEALE]
    {\includegraphics[width=0.15\textwidth]{top-320-EIEALE.png}}
    \subfigure[WY]
    {\includegraphics[width=0.15\textwidth]{top-320-WY.png}} \\
    \caption{Front view (First row) and vertical view (Second row) of the material interface of 3D Rider-Kothe single vortex test at $t=T/2$ with grid resolution of $32 \times 32 \times 64$.}
    \label{fig:3dsviso1}
\end{figure}
%</fig:3dsviso1>

%<*fig:3dsviso2>
\begin{figure}[htbp]
    \centering
    {\includegraphics[width=0.15\textwidth]{sv-front-exact-1.png}}
    {\includegraphics[width=0.15\textwidth]{front-640-EI.png}}
    {\includegraphics[width=0.15\textwidth]{front-640-LE.png}}
    {\includegraphics[width=0.15\textwidth]{front-640-EILE3D.png}}
    {\includegraphics[width=0.15\textwidth]{front-640-EILE3DS.png}}
    {\includegraphics[width=0.15\textwidth]{front-640-EIEALE.png}}
    {\includegraphics[width=0.15\textwidth]{front-640-WY.png}} \\

    \subfigure[Exact]
    {\includegraphics[width=0.15\textwidth]{sv-top-exact-1.png}}
    \subfigure[EI]
    {\includegraphics[width=0.15\textwidth]{top-640-EI.png}}
    \subfigure[LE]
    {\includegraphics[width=0.15\textwidth]{top-640-LE.png}}
    \subfigure[EILE3D]
    {\includegraphics[width=0.15\textwidth]{top-640-EILE3D.png}}
    \subfigure[EILE3DS]
    {\includegraphics[width=0.15\textwidth]{top-640-EILE3DS.png}}
    \subfigure[EIEALE]
    {\includegraphics[width=0.15\textwidth]{top-640-EIEALE.png}}
    \subfigure[WY]
    {\includegraphics[width=0.15\textwidth]{top-640-WY.png}} \\
    \caption{Front view (First row) and vertical view (Second row) of the material interface of 3D Rider-Kothe single vortex test at $t=T$ with grid resolution of $32 \times 32 \times 64$.}
    \label{fig:3dsviso2}
\end{figure}
%</fig:3dsviso2>

%<*fig:3drviso1>
\begin{figure}[htbp]
    \centering
    {\includegraphics[width=0.15\textwidth]{rv-front-exact-2.png}}
    {\includegraphics[width=0.15\textwidth]{front-640-EI.png}}
    {\includegraphics[width=0.15\textwidth]{front-640-LE.png}}
    {\includegraphics[width=0.15\textwidth]{front-640-EILE3D.png}}
    {\includegraphics[width=0.15\textwidth]{front-640-EILE3DS.png}}
    {\includegraphics[width=0.15\textwidth]{front-640-EIEALE.png}}
    {\includegraphics[width=0.15\textwidth]{front-640-WY.png}} \\

    \subfigure[Exact]
    {\includegraphics[width=0.15\textwidth]{rv-top-exact-2.png}}
    \subfigure[EI]
    {\includegraphics[width=0.15\textwidth]{top-640-EI.png}}
    \subfigure[LE]
    {\includegraphics[width=0.15\textwidth]{top-640-LE.png}}
    \subfigure[EILE3D]
    {\includegraphics[width=0.15\textwidth]{top-640-EILE3D.png}}
    \subfigure[EILE3DS]
    {\includegraphics[width=0.15\textwidth]{top-640-EILE3DS.png}}
    \subfigure[EIEALE]
    {\includegraphics[width=0.15\textwidth]{top-640-EIEALE.png}}
    \subfigure[WY]
    {\includegraphics[width=0.15\textwidth]{top-640-WY.png}} \\
    \caption{Front view (First row) and vertical view (Second row) of the material interface of 3D reversed vortex test at $t=T/2$ with grid resolution of $64 \times 64 \times 64$.}
    \label{fig:3drviso1}
\end{figure}
%</fig:3drviso1>

%<*fig:3drviso2>
\begin{figure}[htbp]
    \centering
    {\includegraphics[width=0.15\textwidth]{rv-front-exact-1.png}}
    {\includegraphics[width=0.15\textwidth]{front-1280-EI.png}}
    {\includegraphics[width=0.15\textwidth]{front-1280-LE.png}}
    {\includegraphics[width=0.15\textwidth]{front-1280-EILE3D.png}}
    {\includegraphics[width=0.15\textwidth]{front-1280-EILE3DS.png}}
    {\includegraphics[width=0.15\textwidth]{front-1280-EIEALE.png}}
    {\includegraphics[width=0.15\textwidth]{front-1280-WY.png}} \\

    \subfigure[Exact]
    {\includegraphics[width=0.15\textwidth]{rv-top-exact-1.png}}
    \subfigure[EI]
    {\includegraphics[width=0.15\textwidth]{top-1280-EI.png}}
    \subfigure[LE]
    {\includegraphics[width=0.15\textwidth]{top-1280-LE.png}}
    \subfigure[EILE3D]
    {\includegraphics[width=0.15\textwidth]{top-1280-EILE3D.png}}
    \subfigure[EILE3DS]
    {\includegraphics[width=0.15\textwidth]{top-1280-EILE3DS.png}}
    \subfigure[EIEALE]
    {\includegraphics[width=0.15\textwidth]{top-1280-EIEALE.png}}
    \subfigure[WY]
    {\includegraphics[width=0.15\textwidth]{top-1280-WY.png}} \\
    \caption{Front view (First row) and vertical view (Second row) of the material interface of 3D reversed vortex test at $t=T$ with grid resolution of $64 \times 64 \times 64$.}
    \label{fig:3drviso2}
\end{figure}
%</fig:3drviso2>

% %<*fig:3drviso2>
% \begin{figure}[htbp]
%     \centering
%     {\includegraphics[width=0.15\textwidth]{figures/reversevortex/front-exact-1.png}}
%     {\includegraphics[width=0.15\textwidth]{figures/reversevortex/front-1280-EI.png}}
%     {\includegraphics[width=0.15\textwidth]{figures/reversevortex/front-1280-LE.png}}
%     {\includegraphics[width=0.15\textwidth]{figures/reversevortex/front-1280-EILE3D.png}}
%     {\includegraphics[width=0.15\textwidth]{figures/reversevortex/front-1280-EILE3DS.png}}
%     {\includegraphics[width=0.15\textwidth]{figures/reversevortex/front-1280-EIEALE.png}}
%     {\includegraphics[width=0.15\textwidth]{figures/reversevortex/front-1280-WY.png}} \\

%     \subfigure[Exact]
%     {\includegraphics[width=0.15\textwidth]{figures/reversevortex/top-exact-1.png}}
%     % \subfigure[EI]
%     % {\includegraphics[width=0.15\textwidth]{figures/reversevortex/top-640-EI.png}}
%     \subfigure[LE]
%     {\includegraphics[width=0.15\textwidth]{figures/reversevortex/top-640-LE.png}}
%     \subfigure[EILE3D]
%     {\includegraphics[width=0.15\textwidth]{figures/reversevortex/top-640-EILE3D.png}}
%     \subfigure[EILE3DS]
%     {\includegraphics[width=0.15\textwidth]{figures/reversevortex/top-640-EILE3DS.png}}
%     \subfigure[EIEALE]
%     {\includegraphics[width=0.15\textwidth]{figures/reversevortex/top-640-EIEALE.png}}
%     \subfigure[WY]
%     {\includegraphics[width=0.15\textwidth]{figures/reversevortex/top-640-WY.png}} \\
%     \caption{(a) Geometric error and (b) mass error of 3D reversed vortex test with the change of CFL number on a $64 \times 64 \times 64$ mesh. The correponding data in shown in Table \ref{tab:3drvresos} and Table \ref{tab:3drvresosmass}.}
%     \label{fig:3drviso2}
% \end{figure}
 %</fig:3drviso2>


==> tables.tex <==

%<*tab:comparemethods2d>
\begin{table}[htbp]
    \centering
    \caption{Summary of 2D advection methods,
        where $P_1$ indicates the global mass conservation condition, \smallskip
        $P_2$ indicates the local bound condition, \smallskip
        $P_3$ indicates the global geometrical consistency condition, \smallskip
        $n_s$ is the split advection sweep per full advection step.}
    \label{tab:comparemethods2d}
    \begin{tabular}{llllll}
        \toprule
        Method & $P_1$      & $P_2$      & $P_3$      & $n_s$ & CFL limit \\ \midrule
        EI     & $\times$   & $\bigcirc$ & $\times$   & 2     & 1/2       \\ \hline
        LE     & $\times$   & $\bigcirc$ & $\times$   & 2     & 1/2       \\ \hline
        EILE2D & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & 2     & 1/2       \\ \hline
        LEEI2D & $\times$   & $\bigcirc$ & $\times$   & 2     & 1/2       \\ \hline
        WY     & $\bigcirc$ & $\bigcirc$ & $\times$   & 2     & 1/4       \\ \bottomrule
    \end{tabular}
\end{table}
%</tab:comparemethods2d>

%<*tab:comparemethods3d>
\begin{table}[htbp]
    \centering
    \caption{Summary of 3D advection methods,
        where $P_1$ indicates the global mass conservation condition, \smallskip
        $P_2$ indicates the local bound condition, \smallskip
        $P_3$ indicates the global geometrical consistency condition, \smallskip
        $n_s$ is the split advection sweep per full advection step.}
    \label{tab:comparemethods3d}
    \begin{tabular}{llllll}
        \toprule
        Method   & $P_1$      & $P_2$          & $P_3$      & $n_s$ & CFL limit \\ \midrule
        EI       & $\times$   & $\bigcirc$     & $\times$   & 3     & 1/2       \\ \hline
        LE       & $\times$   & $\bigcirc$     & $\times$   & 3     & 1/2       \\ \hline
        EILE3D   & $\bigcirc$ & $\bigcirc$     & $\bigcirc$ & 6     & 1 (?)     \\ \hline
        EILE3DS  & $\times$   & $\bigcirc$     & $\times$   & 3     & 1/2       \\ \hline
        EI-EA-LE & $\times$   & $\bigcirc$ (?) & $\times$   & 3     & 1/2       \\ \hline
        WY       & $\bigcirc$ & $\bigcirc$     & $\times$   & 3     & 1/6       \\ \bottomrule
    \end{tabular}
\end{table}


%</tab:comparemethods3d>

%<*tab:mappingregion>
\begin{table}
    \centering
    \caption{The areas of the departure and target regions for different split strategy}
    \label{tab:mappingregion}
    \begin{tabular}{llll}
        \toprule
         & $A_{\Omega_d}$                          & ${A_{\Omega_t}}$ & $r = \frac{A_{\Omega_t}}{A_{\Omega_d}}$ \\
        \midrule
        EI
         & $\frac{1}{\beta_x} A_{\Omega_g}$
         & $\frac{1}{\beta_y} a_{\Omega_g}$
         & $\frac{2-\gamma_y}{\gamma_y}$
        \\
        LE
         & $A_{\Omega_g}$
         & $\gamma_x \gamma_y A_{\Omega_g}$
         & $\gamma_y (2-\gamma_y)$
        \\
        LE-EI
         & $A_{\Omega_g}$
         & $\frac{\gamma_y}{\beta_x} A_{\Omega_g}$
         & $\gamma_y^2$                                                                                         \\
        EI-LE
         & $\frac{1}{\beta_x} A_{\Omega_g}$
         & $\gamma_y A_{\Omega_g}$
         & 1                                                                                                    \\
        \bottomrule
    \end{tabular}
\end{table}
%</tab:mappingregion>

%<*tab:cputime>
\begin{table}[htbp]
    \centering
    \caption{CPU time on different 3D advection methods with the two \smallskip
        geometrical algorithm for volume fraction and centroids.}
    \label{tab:cputime}

    \begin{tabular}{@{}lllllll@{}}
        \toprule
        Geometrical method                                                  & EI                     & LE                     & EILE3D                 & EILE3DS                & EIEALE                 & WY                     \\ \midrule
        \multirow{3}{*}{Current algorithm}                                  & 47.27                  & 47.42                  & 123.96                 & 45.16                  & 50.64                  & 51.96                  \\
                                                                            & \textit{3.95}          & \textit{3.59}          & \textit{7.93}          & \textit{3.75}          & \textit{3.94}          & \textit{4.29}          \\
                                                                            & \textit{\textbf{0.08}} & \textit{\textbf{0.08}} & \textit{\textbf{0.06}} & \textit{\textbf{0.08}} & \textit{\textbf{0.08}} & \textit{\textbf{0.08}} \\ \midrule
        \multirow{3}{*}{Geometrical algorithm \citep{jemison_coupled_2013}} & 255.02                 & 276.47                 & 619.20                 & 259.89                 & 287.67                 & 289.61                 \\
                                                                            & \textit{201.82}        & \textit{214.20}        & \textit{474.40}        & \textit{203.40}        & \textit{221.10}        & \textit{227.20}        \\
                                                                            & \textit{\textbf{0.79}} & \textit{\textbf{0.77}} & \textit{\textbf{0.77}} & \textit{\textbf{0.78}} & \textit{\textbf{0.77}} & \textit{\textbf{0.78}} \\ \midrule
        \multicolumn{7}{l}{* The total CPU times are in normal font between mesh entries.}                                                                                                                                        \\
        \multicolumn{7}{l}{** The CPU times on advection term are in italics between mesh entries.}                                                                                                                               \\
        \multicolumn{7}{l}{*** The ratios of advection time and total CPU time are in bold between mesh entries.}                                                                                                                 \\ \bottomrule
    \end{tabular}
\end{table}

%</tab:cputime>


%<*tab:2dzalesakcfls>
\begin{table}[htbp]
    \centering
    \caption{Geometrical errors in 2D Zalesak's disk rotation test when CFL number is 0.05 and 0.05, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:2dzalesakcfls}(a) and Fig. \ref{fig:2dzalesakcfls}(b)}
    \label{tab:2dzalesakcfls}

    \begin{tabular}{@{}llllll@{}}
        \toprule
        Resolution ($N$)     & EI            & LE            & LEEI2D        & EILE2D        & WY            \\ \midrule
        \multicolumn{6}{l}{$\rm{CFL}=0.05$}                                                                  \\ \midrule
        \multirow{2}{*}{16}  & 1.37E-02      & 1.37E-02      & 1.37E-02      & 1.37E-02      & 1.38E-02      \\
                             & \textit{2.19} & \textit{2.19} & \textit{2.19} & \textit{2.19} & \textit{2.20} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{32}  & 3.00E-03      & 3.00E-03      & 3.00E-03      & 3.00E-03      & 3.00E-03      \\
                             & \textit{1.40} & \textit{1.41} & \textit{1.41} & \textit{1.40} & \textit{1.40} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{64}  & 1.14E-03      & 1.13E-03      & 1.13E-03      & 1.14E-03      & 1.14E-03      \\
                             & \textit{1.08} & \textit{1.13} & \textit{1.08} & \textit{1.09} & \textit{1.07} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{128} & 5.38E-04      & 5.19E-04      & 5.36E-04      & 5.34E-04      & 5.39E-04      \\
                             & \textit{0.75} & \textit{0.64} & \textit{0.67} & \textit{0.73} & \textit{0.74} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        128                  & 3.20E-04      & 3.34E-04      & 3.37E-04      & 3.22E-04      & 3.22E-04      \\
                             &               &               &               &               &               \\ \midrule
        \multicolumn{6}{l}{$\rm{CFL}=0.5$}                                                                   \\ \midrule
        \multirow{2}{*}{16}  & 1.10E-02      & 1.10E-02      & 1.10E-02      & 1.10E-02      & 1.10E-02      \\
                             & \textit{2.03} & \textit{2.02} & \textit{2.02} & \textit{2.03} & \textit{2.02} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{32}  & 2.70E-03      & 2.70E-03      & 2.70E-03      & 2.70E-03      & 2.70E-03      \\
                             & \textit{1.35} & \textit{1.35} & \textit{1.35} & \textit{1.35} & \textit{1.35} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{64}  & 1.06E-03      & 1.06E-03      & 1.06E-03      & 1.06E-03      & 1.06E-03      \\
                             & \textit{1.47} & \textit{1.47} & \textit{1.47} & \textit{1.47} & \textit{1.47} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{128} & 3.83E-04      & 3.83E-04      & 3.83E-04      & 3.83E-04      & 3.83E-04      \\
                             & \textit{1.39} & \textit{1.39} & \textit{1.39} & \textit{1.39} & \textit{1.39} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        256                  & 1.46E-04      & 1.46E-04      & 1.46E-04      & 1.46E-04      & 1.46E-04      \\
                             &               &               &               &               &               \\ \midrule
        \multicolumn{6}{l}{The computed orders of accuracy are in italics between mesh entries.}             \\ \bottomrule
    \end{tabular}


\end{table}
%</tab:2dzalesakcfls>


%<*tab:2dsvcfls>
\begin{table}[ht]
    \centering
    \caption{Geometrical errors in 2D Rider-Kothe single vortex test when CFL number is 0.05 and 1.0, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:2dsvcfls}(a) and Fig. \ref{fig:2dsvcfls}(c)}
    \label{tab:2dsvcfls}

    \begin{tabular}{@{}llllll@{}}
        \toprule
        Resolution ($N$)     & EI            & LE            & LEEI2D        & EILE2D        & WY            \\ \midrule
        \multicolumn{6}{l}{$\rm{CFL}=0.05$}                                                                  \\ \midrule
        \multirow{2}{*}{16}  & 7.93E-02      & 6.39E-02      & 6.82E-02      & 6.15E-02      & 8.04E-02      \\
                             & \textit{1.35} & \textit{0.98} & \textit{1.09} & \textit{0.62} & \textit{1.37} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{32}  & 3.11E-02      & 3.23E-02      & 3.20E-02      & 4.00E-02      & 3.12E-02      \\
                             & \textit{1.94} & \textit{1.80} & \textit{1.88} & \textit{2.11} & \textit{1.49} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{64}  & 8.08E-03      & 9.28E-03      & 8.68E-03      & 9.29E-03      & 1.11E-02      \\
                             & \textit{1.15} & \textit{1.08} & \textit{1.44} & \textit{1.34} & \textit{1.72} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{128} & 3.64E-03      & 4.39E-03      & 3.20E-03      & 3.68E-03      & 3.37E-03      \\
                             & \textit{1.80} & \textit{1.96} & \textit{1.61} & \textit{1.97} & \textit{1.31} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        256                  & 1.05E-03      & 1.13E-03      & 1.05E-03      & 9.41E-04      & 1.36E-03      \\
                             &               &               &               &               &               \\ \midrule
        \multicolumn{6}{l}{$\rm{CFL}=1.0$}                                                                   \\ \midrule
        \multirow{2}{*}{16}  & 7.99E-02      & 5.85E-02      & 7.68E-02      & 7.72E-02      & 8.16E-02      \\
                             & \textit{0.54} & \textit{0.70} & \textit{1.29} & \textit{1.34} & \textit{1.02} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{32}  & 5.48E-02      & 3.61E-02      & 3.13E-02      & 3.04E-02      & 4.02E-02      \\
                             & \textit{1.06} & \textit{0.76} & \textit{1.89} & \textit{1.78} & \textit{1.17} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{64}  & 2.64E-02      & 2.13E-02      & 8.47E-03      & 8.83E-03      & 1.79E-02      \\
                             & \textit{1.11} & \textit{1.05} & \textit{1.58} & \textit{1.57} & \textit{0.91} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{128} & 1.22E-02      & 1.03E-02      & 2.83E-03      & 2.98E-03      & 9.52E-03      \\
                             & \textit{1.00} & \textit{1.03} & \textit{1.18} & \textit{1.23} & \textit{1.05} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        256                  & 6.12E-03      & 5.05E-03      & 1.25E-03      & 1.27E-03      & 4.59E-03      \\
                             &               &               &               &               &               \\ \midrule
        \multicolumn{6}{l}{The computed orders of accuracy are in italics between mesh entries.}             \\ \bottomrule
    \end{tabular}
\end{table}

%</tab:2dsvcfls>


%<*tab:2drvcfls>
\begin{table}[ht]
    \centering
    \caption{Geometrical errors in 2D reversed vortex test when CFL number is 0.05 and 1.0, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:2drvcfls}(a) and Fig. \ref{fig:2drvcfls}(c)}
    \label{tab:2drvcfls}

    \begin{tabular}{@{}llllll@{}}
        \toprule
        Resolution ($N$)     & EI            & LE            & LEEI2D        & EILE2D        & WY            \\ \midrule
        \multicolumn{6}{l}{$\rm{CFL}=0.05$}                                                                  \\ \midrule
        \multirow{2}{*}{16}  & 1.80E-02      & 1.52E-02      & 1.62E-02      & 1.57E-02      & 2.24E-02      \\
                             & \textit{0.98} & \textit{1.10} & \textit{1.10} & \textit{1.04} & \textit{1.55} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{32}  & 9.13E-03      & 7.08E-03      & 7.55E-03      & 7.64E-03      & 7.66E-03      \\
                             & \textit{0.39} & \textit{0.14} & \textit{0.30} & \textit{0.28} & \textit{0.38} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{64}  & 6.96E-03      & 6.41E-03      & 6.12E-03      & 6.27E-03      & 5.88E-03      \\
                             & \textit{0.30} & \textit{0.23} & \textit{0.18} & \textit{0.20} & \textit{0.08} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{128} & 5.67E-03      & 5.45E-03      & 5.41E-03      & 5.45E-03      & 5.55E-03      \\
                             & \textit{1.60} & \textit{1.63} & \textit{1.63} & \textit{1.59} & \textit{1.44} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        256                  & 1.87E-03      & 1.76E-03      & 1.75E-03      & 1.81E-03      & 2.05E-03      \\
                             &               &               &               &               &               \\ \midrule
        \multicolumn{6}{l}{$\rm{CFL}=1.0$}                                                                   \\ \midrule
        \multirow{2}{*}{16}  & 8.72E-02      & 2.71E-02      & 1.31E-02      & 3.24E-02      & 4.44E-02      \\
                             & \textit{0.80} & \textit{0.24} & \textit{0.58} & \textit{1.30} & \textit{0.69} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{32}  & 5.01E-02      & 2.29E-02      & 8.72E-03      & 1.32E-02      & 2.75E-02      \\
                             & \textit{0.92} & \textit{0.64} & \textit{0.29} & \textit{0.36} & \textit{0.95} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{64}  & 2.65E-02      & 1.47E-02      & 7.13E-03      & 1.02E-02      & 1.43E-02      \\
                             & \textit{0.74} & \textit{0.66} & \textit{0.20} & \textit{0.44} & \textit{0.72} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        \multirow{2}{*}{128} & 1.59E-02      & 9.32E-03      & 6.20E-03      & 7.57E-03      & 8.69E-03      \\
                             & \textit{1.29} & \textit{0.94} & \textit{1.57} & \textit{1.68} & \textit{1.24} \\
                             & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     \\
        256                  & 6.49E-03      & 4.87E-03      & 2.09E-03      & 2.35E-03      & 3.68E-03      \\
                             &               &               &               &               &               \\ \midrule
        \multicolumn{6}{l}{The computed orders of accuracy are in italics between mesh entries.}             \\ \bottomrule
    \end{tabular}
\end{table}

%</tab:2drvcfls>

%<*tab:2dsvcflsmass>
\begin{table}[ht]
    \centering
    \caption{Mass errors in 2D Rider-Kothe single vortex test when CFL number is 0.05 and 1.0, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:2dsvcfls}(b) and Fig. \ref{fig:2dsvcfls}(d)}
    \label{tab:2dsvcflsmass}

    \begin{tabular}{@{}llllll@{}}
        \toprule
        Resolution ($N$) & EI       & LE        & LEEI2D    & EILE2D   & WY       \\ \midrule
        \multicolumn{6}{l}{$\rm{CFL}=0.05$}                                       \\ \midrule
        16               & 1.19E-02 & -1.23E-02 & -3.67E-04 & 5.85E-14 & 1.24E-13 \\
        32               & 5.42E-03 & -5.40E-03 & -1.24E-04 & 2.62E-13 & 2.13E-13 \\
        64               & 2.70E-03 & -2.68E-03 & 5.00E-06  & 3.21E-13 & 3.19E-13 \\
        128              & 1.35E-03 & -1.34E-03 & 8.00E-06  & 2.24E-13 & 2.93E-13 \\
        256              & 6.76E-04 & -6.72E-04 & 3.00E-06  & 3.58E-13 & 3.15E-13 \\ \midrule
        \multicolumn{6}{l}{$\rm{CFL}=1.0$}                                        \\ \midrule
        16               & 2.32E-01 & -2.02E-01 & -2.13E-02 & 3.73E-15 & 8.64E-15 \\
        32               & 1.07E-01 & -9.56E-02 & -1.48E-03 & 1.06E-14 & 1.24E-14 \\
        64               & 5.35E-02 & -4.93E-02 & -5.40E-05 & 5.89E-15 & 1.63E-14 \\
        128              & 2.69E-02 & -2.58E-02 & 6.80E-05  & 1.14E-14 & 1.90E-14 \\
        256              & 1.35E-02 & -1.32E-02 & 5.10E-05  & 9.62E-15 & 2.08E-14 \\ \bottomrule
    \end{tabular}
\end{table}
%</tab:2dsvcflsmass>

%<*tab:2drvcflsmass>
\begin{table}[ht]
    \centering
    \caption{Mass errors in 2D reversed vortex test when CFL number is 0.05 and 1.0, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:2drvcfls}(b) and Fig. \ref{fig:2drvcfls}(d)}
    \label{tab:2drvcflsmass}
    \begin{tabular}{@{}llllll@{}}
        \toprule
        Resolution ($N$) & EI        & LE        & LEEI2D    & EILE2D   & WY        \\ \midrule
        \multicolumn{6}{l}{$\rm{CFL}=0.05$}                                         \\ \midrule
        16               & 2.61E-03  & -2.34E-03 & 1.92E-03  & 5.89E-15 & 1.49E-14  \\
        32               & -3.34E-03 & 3.28E-03  & 7.42E-04  & 1.65E-14 & 3.46E-14  \\
        64               & -1.90E-03 & 1.77E-03  & -1.10E-05 & 1.63E-14 & 1.06E-14  \\
        128              & -9.91E-04 & 9.66E-04  & 1.20E-05  & 1.63E-14 & 1.98E-14  \\
        256              & -5.26E-04 & 5.49E-04  & 3.50E-05  & 2.75E-14 & 3.30E-14  \\ \midrule
        \multicolumn{6}{l}{$\rm{CFL}=1.0$}                                          \\ \midrule
        16               & -6.13E-01 & -1.49E-01 & -6.26E-02 & 9.82E-16 & -3.23E-03 \\
        32               & -1.94E-01 & -1.52E-02 & -8.40E-03 & 1.96E-15 & 2.04E-03  \\
        64               & -6.75E-02 & 1.15E-02  & -4.57E-03 & 1.96E-15 & 1.27E-03  \\
        128              & -2.65E-02 & 1.16E-02  & -7.68E-04 & 1.96E-16 & 2.41E-04  \\
        256              & -1.28E-02 & 8.58E-03  & 3.37E-04  & 1.77E-15 & 1.85E-04  \\ \bottomrule
    \end{tabular}
\end{table}
%</tab:2drvcflsmass>

%<*tab:2dzalesakresos>
\begin{table}[ht]
    \centering
    \caption{Geometrical errors in 2D Zalesak's disk rotation test with a $64 \times 64$ mesh, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:2dzalesakresos}}
    \label{tab:2dzalesakresos}
    \begin{tabular}{@{}llllll@{}}
        \toprule
        CFL number & EI       & LE       & LEEI2D   & EILE2D   & WY       \\ \midrule
        0.05       & 1.14E-03 & 1.13E-03 & 1.13E-03 & 1.14E-03 & 1.14E-03 \\
        0.1        & 1.13E-03 & 1.13E-03 & 1.13E-03 & 1.13E-03 & 1.13E-03 \\
        0.15       & 1.12E-03 & 1.12E-03 & 1.12E-03 & 1.12E-03 & 1.12E-03 \\
        0.2        & 1.11E-03 & 1.11E-03 & 1.11E-03 & 1.11E-03 & 1.11E-03 \\
        0.25       & 1.11E-03 & 1.11E-03 & 1.11E-03 & 1.11E-03 & 1.11E-03 \\
        0.3        & 1.10E-03 & 1.10E-03 & 1.10E-03 & 1.10E-03 & 1.10E-03 \\
        0.5        & 1.06E-03 & 1.06E-03 & 1.06E-03 & 1.06E-03 & 1.06E-03 \\ \bottomrule
    \end{tabular}
\end{table}
%</tab:2dzalesakresos>

%<*tab:2dsvresos>
\begin{table}[ht]
    \centering
    \caption{Geometrical errors in 2D Rider-Kothe single vortex test with a $64 \times 64$ mesh, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:2dsvresos} (a)}
    \label{tab:2dsvresos}
    \begin{tabular}{@{}llllll@{}}
        \toprule
        CFL number & EI       & LE       & LEEI2D   & EILE2D   & WY       \\ \midrule
        0.05       & 8.08E-03 & 9.28E-03 & 8.68E-03 & 9.29E-03 & 1.11E-02 \\
        0.1        & 8.51E-03 & 7.88E-03 & 8.08E-03 & 7.68E-03 & 9.46E-03 \\
        0.15       & 8.35E-03 & 7.68E-03 & 7.18E-03 & 6.45E-03 & 9.51E-03 \\
        0.2        & 9.13E-03 & 8.49E-03 & 6.19E-03 & 7.19E-03 & 9.69E-03 \\
        0.25       & 1.01E-02 & 9.46E-03 & 6.39E-03 & 7.16E-03 & 1.02E-02 \\
        0.3        & 1.16E-02 & 9.96E-03 & 6.42E-03 & 6.66E-03 & 1.07E-02 \\
        0.5        & 1.52E-02 & 1.33E-02 & 7.01E-03 & 7.23E-03 & 1.22E-02 \\
        0.8        & 2.22E-02 & 1.81E-02 & 7.63E-03 & 8.02E-03 & 1.59E-02 \\
        1.0        & 2.64E-02 & 2.13E-02 & 8.47E-03 & 8.83E-03 & 1.79E-02 \\ \bottomrule
    \end{tabular}
\end{table}
%</tab:2dsvresos>

%<*tab:2drvresos>
\begin{table}[ht]
    \centering
    \caption{Geometrical errors reconstruction in 2D reversed vortex test with a $64 \times 64$ mesh, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:2drvresos} (b)}
    \label{tab:2drvresos}

    \begin{tabular}{@{}llllll@{}}
        \toprule
        CFL number & EI       & LE       & LEEI2D   & EILE2D   & WY       \\ \midrule
        0.05       & 6.96E-03 & 6.41E-03 & 6.12E-03 & 6.27E-03 & 5.88E-03 \\
        0.1        & 8.03E-03 & 6.97E-03 & 6.31E-03 & 6.55E-03 & 6.02E-03 \\
        0.15       & 8.78E-03 & 7.38E-03 & 5.92E-03 & 6.45E-03 & 6.22E-03 \\
        0.2        & 9.93E-03 & 6.82E-03 & 6.37E-03 & 6.71E-03 & 6.69E-03 \\
        0.25       & 1.10E-02 & 7.60E-03 & 6.47E-03 & 7.35E-03 & 7.09E-03 \\
        0.3        & 1.22E-02 & 7.30E-03 & 6.54E-03 & 7.85E-03 & 7.80E-03 \\
        0.5        & 1.57E-02 & 9.41E-03 & 6.46E-03 & 8.09E-03 & 9.10E-03 \\
        0.8        & 2.25E-02 & 1.26E-02 & 6.38E-03 & 9.11E-03 & 1.18E-02 \\
        1.0        & 2.65E-02 & 1.47E-02 & 7.13E-03 & 1.02E-02 & 1.43E-02 \\ \bottomrule
    \end{tabular}
\end{table}

%</tab:2drvresos>

%<*tab:2dsvresosmass>
\begin{table}[ht]
    \centering
    \caption{Mass errors in 2D Rider-Kothe single vortex test with a $64 \times 64$ mesh, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:2dsvresos}(b)}
    \label{tab:2dsvresosmass}
    \begin{tabular}{@{}llllll@{}}
        \toprule
        CFL number & EI       & LE        & LEEI2D    & EILE2D   & WY       \\ \midrule
        0.05       & 2.70E-03 & -2.68E-03 & 5.00E-06  & 3.21E-13 & 3.19E-13 \\
        0.1        & 5.40E-03 & -5.33E-03 & 2.20E-05  & 1.37E-13 & 1.56E-13 \\
        0.15       & 8.09E-03 & -7.97E-03 & 3.00E-05  & 9.13E-14 & 1.07E-13 \\
        0.2        & 1.08E-02 & -1.06E-02 & 2.90E-05  & 5.30E-14 & 8.01E-14 \\
        0.25       & 1.35E-02 & -1.32E-02 & 2.70E-05  & 4.71E-14 & 6.52E-14 \\
        0.3        & 1.61E-02 & -1.58E-02 & 2.60E-05  & 1.08E-14 & 5.42E-14 \\
        0.5        & 2.69E-02 & -2.58E-02 & 2.10E-05  & 2.32E-14 & 3.20E-14 \\
        0.8        & 4.29E-02 & -4.02E-02 & -9.60E-05 & 1.51E-14 & 2.18E-14 \\
        1          & 5.35E-02 & -4.93E-02 & -5.40E-05 & 5.89E-15 & 1.63E-14 \\ \bottomrule
    \end{tabular}
\end{table}

%</tab:2dsvresosmass>

%<*tab:2drvresosmass>
\begin{table}[ht]
    \centering
    \caption{Mass errors in 2D reversed vortex test with a $64 \times 64$ mesh, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:2drvresos}(b)}
    \label{tab:2drvresosmass}
    \begin{tabular}{@{}llllll@{}}
        \toprule
        CFL number & EI        & LE       & LEEI2D    & EILE2D    & WY        \\ \midrule
        0.05       & -1.90E-03 & 1.77E-03 & -1.10E-05 & 1.63E-14  & 1.06E-14  \\
        0.1        & -4.01E-03 & 3.35E-03 & -1.40E-04 & -5.10E-15 & 6.68E-15  \\
        0.15       & -6.10E-03 & 4.79E-03 & -8.60E-05 & -3.97E-14 & 5.10E-15  \\
        0.2        & -8.47E-03 & 6.65E-03 & -2.80E-04 & 4.71E-15  & 5.69E-15  \\
        0.25       & -1.08E-02 & 7.91E-03 & -5.23E-04 & 5.50E-15  & 5.10E-15  \\
        0.3        & -1.37E-02 & 9.33E-03 & -4.07E-04 & 3.73E-15  & 5.10E-15  \\
        0.5        & -2.58E-02 & 1.23E-02 & -9.80E-04 & 2.75E-15  & 3.93E-15  \\
        0.8        & -4.71E-02 & 1.33E-02 & -2.72E-03 & 7.85E-16  & -2.33E-05 \\
        1          & -6.75E-02 & 1.15E-02 & -4.57E-03 & 1.96E-15  & 1.27E-03  \\ \bottomrule
    \end{tabular}
\end{table}

%</tab:2drvresosmass>


%<*tab:3dzalesakcfls>
\begin{table}[ht]
    \centering
    \caption{Geometrical errors in 3D Zalesak's test when CFL number is 0.3, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:3dzalesakcfls}}
    \label{tab:3dzalesakcfls}
    \begin{tabular}{@{}lllllll@{}}
        \toprule
        Resolution ($N$)    & \textbf{EI}   & \textbf{LE}   & \textbf{EILE3D} & \textbf{EILE3DS} & \textbf{EIEALE} & \textbf{WY}   \\ \midrule
        \multirow{2}{*}{16} & 1.23E-02      & 1.23E-02      & 1.27E-02        & 1.23E-02         & 1.22E-02        & 1.22E-02      \\
                            & \textit{1.54} & \textit{1.54} & \textit{1.52}   & \textit{1.54}    & \textit{1.53}   & \textit{1.53} \\
                            & \textit{}     & \textit{}     & \textit{}       & \textit{}        & \textit{}       &               \\
        \multirow{2}{*}{32} & 4.22E-03      & 4.22E-03      & 4.46E-03        & 4.22E-03         & 4.23E-03        & 4.23E-03      \\
                            & \textit{1.73} & \textit{1.73} & \textit{1.73}   & \textit{1.73}    & \textit{1.74}   & \textit{1.74} \\
                            & \textit{}     & \textit{}     & \textit{}       & \textit{}        & \textit{}       &               \\
        \multirow{2}{*}{64} & 1.27E-03      & 1.27E-03      & 1.35E-03        & 1.27E-03         & 1.27E-03        & 1.27E-03      \\
                            & \textit{1.08} & \textit{1.08} & \textit{0.97}   & \textit{1.08}    & \textit{1.07}   & \textit{1.07} \\
                            & \textit{}     & \textit{}     & \textit{}       & \textit{}        & \textit{}       &               \\
        128                 & 6.03E-04      & 6.03E-04      & 6.86E-04        & 6.03E-04         & 6.02E-04        & 6.02E-04      \\
                            &               &               &                 &                  &                 &               \\ \midrule
        \multicolumn{7}{l}{The computed orders of accuracy are in italics between mesh entries.}                                   \\ \bottomrule
    \end{tabular}
\end{table}
%</tab:3dzalesakcfls>

%<*tab:3dsvcfls>
\begin{table}[ht]
    \centering
    \caption{Geometrical errors in 3D single vortex test with a $64 \times 64 \times 64$ mesh, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:3dsvcfls} (a) and Fig. \ref{fig:3dsvcfls} (c)}
    \label{tab:3dsvcfls}

    \begin{tabular}{@{}lllllll@{}}
        \toprule
        Resolution ($N$)    & EI            & LE            & EILE3D        & EILE3DS       & EIEALE        & WY            \\ \midrule
        \multicolumn{7}{l}{$\rm{CFL}=0.3$}                                                                                  \\ \midrule
        \multirow{2}{*}{16} & 9.68E-03      & 9.85E-03      & 1.01E-02      & 1.11E-02      & 1.18E-02      & 9.37E-03      \\
                            & \textit{0.20} & \textit{0.60} & \textit{0.53} & \textit{0.75} & \textit{0.85} & \textit{0.49} \\
                            & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     &               \\
        \multirow{2}{*}{32} & 8.45E-03      & 6.50E-03      & 6.98E-03      & 6.60E-03      & 6.54E-03      & 6.67E-03      \\
                            & \textit{0.67} & \textit{0.95} & \textit{1.16} & \textit{1.01} & \textit{0.97} & \textit{0.97} \\
                            & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     &               \\
        \multirow{2}{*}{64} & 5.30E-03      & 3.36E-03      & 3.12E-03      & 3.27E-03      & 3.34E-03      & 3.40E-03      \\
                            & \textit{0.96} & \textit{1.15} & \textit{1.18} & \textit{1.25} & \textit{1.28} & \textit{1.29} \\
                            & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     &               \\
        128                 & 2.73E-03      & 1.51E-03      & 1.37E-03      & 1.37E-03      & 1.38E-03      & 1.39E-03      \\
                            &               &               &               &               &               &               \\ \midrule
        \multicolumn{7}{l}{$\rm{CFL}=1.0$}                                                                                  \\ \midrule
        \multirow{2}{*}{16} & 1.04E-02      & 1.24E-02      & 1.05E-01      & 1.19E-02      & 1.14E-02      & 1.14E-02      \\
                            & \textit{0.02} & \textit{0.74} & \textit{0.27} & \textit{0.67} & \textit{0.58} & \textit{0.56} \\
                            & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     &               \\
        \multirow{2}{*}{32} & 1.02E-02      & 7.47E-03      & 8.72E-02      & 7.48E-03      & 7.57E-03      & 7.74E-03      \\
                            & \textit{0.47} & \textit{0.84} & \textit{0.20} & \textit{0.95} & \textit{0.98} & \textit{0.98} \\
                            & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     &               \\
        \multirow{2}{*}{64} & 7.40E-03      & 4.17E-03      & 7.60E-02      & 3.88E-03      & 3.85E-03      & 3.92E-03      \\
                            & \textit{0.82} & \textit{1.03} & \textit{0.10} & \textit{1.13} & \textit{1.09} & \textit{1.11} \\
                            & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     &               \\
        128                 & 4.18E-03      & 2.04E-03      & 7.06E-02      & 1.78E-03      & 1.81E-03      & 1.81E-03      \\
                            &               &               &               &               &               &               \\ \midrule
        \multicolumn{7}{l}{The computed orders of accuracy are in italics between mesh entries.}                            \\ \bottomrule
    \end{tabular}
\end{table}
%</tab:3dsvcfls>

%<*tab:3drvcfls>
\begin{table}[ht]
    \centering
    \caption{Geometrical errors in 3D reversed vortex test with a $64 \times 64 \times 64$ mesh, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:3drvcfls} (a) and Fig. \ref{fig:3drvcfls} (c)}
    \label{tab:3drvcfls}
    \begin{tabular}{@{}lllllll@{}}
        \toprule
        Resolution ($N$)    & EI            & LE            & EILE3D        & EILE3DS       & EIEALE        & WY            \\ \midrule
        \multicolumn{7}{l}{$\rm{CFL}=0.3$}                                                                                  \\ \midrule
        \multirow{2}{*}{16} & 1.11E-02      & 9.83E-03      & 1.03E-02      & 1.04E-02      & 1.04E-02      & 1.06E-02      \\
                            & \textit{0.70} & \textit{0.65} & \textit{0.70} & \textit{0.71} & \textit{0.71} & \textit{0.79} \\
                            & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     &               \\
        \multirow{2}{*}{32} & 6.83E-03      & 6.26E-03      & 6.32E-03      & 6.35E-03      & 6.33E-03      & 6.11E-03      \\
                            & \textit{1.37} & \textit{1.35} & \textit{1.42} & \textit{1.40} & \textit{1.43} & \textit{1.39} \\
                            & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     &               \\
        \multirow{2}{*}{64} & 2.64E-03      & 2.45E-03      & 2.37E-03      & 2.42E-03      & 2.35E-03      & 2.34E-03      \\
                            & \textit{1.85} & \textit{1.96} & \textit{2.10} & \textit{2.02} & \textit{2.11} & \textit{2.10} \\
                            & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     &               \\
        128                 & 7.32E-04      & 6.29E-04      & 5.50E-04      & 5.97E-04      & 5.43E-04      & 5.44E-04      \\
                            &               &               &               &               &               &               \\ \midrule
        \multicolumn{7}{l}{$\rm{CFL}=1.0$}                                                                                  \\ \midrule
        \multirow{2}{*}{16} & 1.35E-02      & 1.23E-02      & 1.04E-02      & 1.15E-02      & 1.07E-02      & 1.10E-02      \\
                            & \textit{0.75} & \textit{0.77} & \textit{0.90} & \textit{0.90} & \textit{0.86} & \textit{0.94} \\
                            & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     &               \\
        \multirow{2}{*}{32} & 8.03E-03      & 7.24E-03      & 5.55E-03      & 6.12E-03      & 5.91E-03      & 5.69E-03      \\
                            & \textit{0.81} & \textit{0.82} & \textit{0.76} & \textit{0.73} & \textit{0.82} & \textit{0.77} \\
                            & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     &               \\
        \multirow{2}{*}{64} & 4.57E-03      & 4.11E-03      & 3.28E-03      & 3.69E-03      & 3.34E-03      & 3.35E-03      \\
                            & \textit{1.30} & \textit{1.36} & \textit{1.53} & \textit{1.44} & \textit{1.54} & \textit{1.54} \\
                            & \textit{}     & \textit{}     & \textit{}     & \textit{}     & \textit{}     &               \\
        256                 & 1.86E-03      & 1.60E-03      & 1.13E-03      & 1.36E-03      & 1.15E-03      & 1.16E-03      \\
                            &               &               &               &               &               &               \\ \midrule
        \multicolumn{7}{l}{The computed orders of accuracy are in italics between mesh entries.}                            \\ \bottomrule
    \end{tabular}
\end{table}
%</tab:3drvcfls>

%<*tab:3dsvcflsmass>
\begin{table}[ht]
    \centering
    \caption{Mass errors in 3D single vortex test when CFL number is 0.05 and 1.0, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:3dsvcfls}(b) and Fig. \ref{fig:3dsvcfls}(d)}
    \label{tab:3dsvcflsmass}

    \begin{tabular}{@{}lllllll@{}}
        \toprule
        Resolution ($N$) & EI       & LE        & EILE3D    & EILE3DS   & EIEALE    & WY        \\ \midrule
        \multicolumn{7}{l}{$\rm{CFL}=0.5$}                                                      \\ \midrule
        16               & 5.34E-01 & -5.48E-01 & -1.32E+01 & 5.83E-02  & -3.50E-03 & -6.13E-16 \\
        32               & 2.82E-01 & -2.59E-01 & -1.13E+01 & 1.05E-03  & -6.16E-04 & 6.50E-15  \\
        64               & 1.34E-01 & -1.19E-01 & -1.02E+01 & -8.59E-04 & -1.70E-05 & 1.63E-14  \\
        128              & 6.43E-02 & -5.99E-02 & -9.74E+00 & -2.96E-04 & 3.70E-05  & 3.66E-14  \\ \midrule
        \multicolumn{7}{l}{$\rm{CFL}=1.0$}                                                      \\ \midrule
        16               & 8.26E-01 & 9.04E-02  & -2.86E+01 & 2.53E-01  & -2.71E-02 & -9.19E-02 \\
        32               & 5.46E-01 & -3.09E-01 & -3.09E+01 & 2.59E-02  & -5.68E-03 & 2.59E-03  \\
        64               & 2.67E-01 & -2.10E-01 & -2.95E+01 & -2.69E-03 & -1.89E-04 & -3.36E-04 \\
        128              & 1.29E-01 & -1.13E-01 & -2.88E+01 & -1.30E-03 & 4.28E-04  & 6.01E-04  \\ \bottomrule
    \end{tabular}
\end{table}
%</tab:3dsvcflsmass>


%<*tab:3drvcflsmass>
\begin{table}[ht]
    \centering
    \caption{Mass errors in 3D reversed vortex test when CFL number is 0.05 and 1.0, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:3drvcfls}(b) and Fig. \ref{fig:3drvcfls}(d)}
    \label{tab:3drvcflsmass}
    \begin{tabular}{@{}lllllll@{}}
        \toprule
        Resolution ($N$) & EI       & LE        & EILE3D   & EILE3DS  & EIEALE    & WY        \\ \midrule
        \multicolumn{7}{l}{$\rm{CFL}=0.3$}                                                    \\ \midrule
        16               & 9.53E-02 & -9.70E-02 & 1.50E-14 & 1.93E-03 & 9.00E-06  & 1.39E-14  \\
        32               & 4.73E-02 & -4.76E-02 & 3.34E-14 & 3.90E-04 & 1.50E-05  & 2.21E-14  \\
        64               & 2.36E-02 & -2.37E-02 & 4.21E-14 & 1.08E-04 & 7.00E-06  & 2.88E-14  \\
        128              & 1.18E-02 & -1.19E-02 & 6.39E-14 & 2.70E-05 & 4.00E-06  & 3.12E-14  \\ \midrule
        \multicolumn{7}{l}{$\rm{CFL}=1.0$}                                                    \\ \midrule
        16               & 2.95E-01 & -3.07E-01 & 7.36E-15 & 2.84E-02 & -2.33E-04 & -6.57E-04 \\
        32               & 1.54E-01 & -1.55E-01 & 1.34E-14 & 5.66E-03 & 5.23E-04  & -2.20E-05 \\
        64               & 7.80E-02 & -7.90E-02 & 1.94E-14 & 1.33E-03 & 3.81E-04  & 1.71E-04  \\
        128              & 3.93E-02 & -3.96E-02 & 7.90E-14 & 3.17E-04 & 2.00E-04  & 1.19E-04  \\ \bottomrule
    \end{tabular}
\end{table}
%</tab:3drvcflsmass>


%<*tab:3dzalesakresos>
\begin{table}[ht]
    \centering
    \caption{Geometrical errors in 3D Zalesak's test with a $64 \times 64 \times 64$ mesh, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:3dzalesakresos}}
    \label{tab:3dzalesakresos}
    \begin{tabular}{@{}lllllll@{}}
        \toprule
             & EI       & LE       & EILE3D   & EILE3DS  & EIEALE   & WY       \\ \midrule
        0.05 & 1.51E-03 & 1.51E-03 & 1.67E-03 & 1.51E-03 & 1.51E-03 & 1.51E-03 \\
        0.1  & 1.40E-03 & 1.40E-03 & 1.51E-03 & 1.40E-03 & 1.40E-03 & 1.40E-03 \\
        0.15 & 1.35E-03 & 1.35E-03 & 1.44E-03 & 1.35E-03 & 1.35E-03 & 1.35E-03 \\
        0.2  & 1.31E-03 & 1.31E-03 & 1.40E-03 & 1.31E-03 & 1.31E-03 & 1.31E-03 \\
        0.25 & 1.29E-03 & 1.29E-03 & 1.37E-03 & 1.29E-03 & 1.29E-03 & 1.29E-03 \\
        0.3  & 1.27E-03 & 1.27E-03 & 1.35E-03 & 1.27E-03 & 1.27E-03 & 1.27E-03 \\
        0.5  & 1.20E-03 & 1.20E-03 & 1.29E-03 & 1.20E-03 & 1.20E-03 & 1.20E-03 \\ \bottomrule
    \end{tabular}
\end{table}
%</tab:3dzalesakresos>


%<*tab:3dsvresos>
\begin{table}[ht]
    \centering
    \caption{Geometrical errors in 3D single vortex test with a $32 \times 32 \times 64$ mesh, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:3dsvresos} (a)}
    \label{tab:3dsvresos}
    \begin{tabular}{@{}lllllll@{}}
        \toprule
        CFL number & EI       & LE       & EILE3D   & EILE3DS  & EIEALE   & WY       \\ \midrule
        0.05       & 3.20E-03 & 3.18E-03 & 2.83E-03 & 3.19E-03 & 3.16E-03 & 3.21E-03 \\
        0.1        & 3.46E-03 & 3.04E-03 & 2.71E-03 & 3.16E-03 & 3.26E-03 & 3.06E-03 \\
        0.15       & 3.91E-03 & 3.20E-03 & 2.87E-03 & 3.00E-03 & 3.11E-03 & 3.14E-03 \\
        0.2        & 4.38E-03 & 3.15E-03 & 3.03E-03 & 3.14E-03 & 3.12E-03 & 3.18E-03 \\
        0.25       & 4.88E-03 & 3.26E-03 & 3.05E-03 & 3.17E-03 & 3.13E-03 & 3.22E-03 \\
        0.3        & 5.30E-03 & 3.36E-03 & 3.12E-03 & 3.27E-03 & 3.34E-03 & 3.40E-03 \\
        0.5        & 7.40E-03 & 4.17E-03 & 7.60E-02 & 3.88E-03 & 3.85E-03 & 3.92E-03 \\
        0.8        & 1.01E-02 & 5.72E-03 & 1.72E-01 & 4.72E-03 & 4.76E-03 & 4.85E-03 \\
        1          & 1.13E-02 & 6.74E-03 & 2.14E-01 & 5.49E-03 & 5.75E-03 & 5.78E-03 \\ \bottomrule
    \end{tabular}
\end{table}
%</tab:3dsvresos>

%<*tab:3drvresos>
\begin{table}[ht]
    \centering
    \caption{Geometrical errors in 3D reversed vortex test with a $64 \times 64 \times 64$ mesh, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:3drvresos} (a)}
    \label{tab:3drvresos}
    \begin{tabular}{@{}lllllll@{}}
        \toprule
        CFL number & EI       & LE       & EILE3D   & EILE3DS  & EIEALE   & WY       \\ \midrule
        0.05       & 2.20E-03 & 2.19E-03 & 2.28E-03 & 2.19E-03 & 2.18E-03 & 2.18E-03 \\
        0.1        & 2.19E-03 & 2.17E-03 & 2.21E-03 & 2.15E-03 & 2.12E-03 & 2.12E-03 \\
        0.15       & 2.31E-03 & 2.26E-03 & 2.19E-03 & 2.20E-03 & 2.18E-03 & 2.18E-03 \\
        0.2        & 2.39E-03 & 2.30E-03 & 2.28E-03 & 2.27E-03 & 2.21E-03 & 2.22E-03 \\
        0.25       & 2.50E-03 & 2.36E-03 & 2.30E-03 & 2.35E-03 & 2.26E-03 & 2.32E-03 \\
        0.3        & 2.64E-03 & 2.45E-03 & 2.37E-03 & 2.42E-03 & 2.35E-03 & 2.34E-03 \\
        0.5        & 3.16E-03 & 2.81E-03 & 2.56E-03 & 2.74E-03 & 2.57E-03 & 2.58E-03 \\
        0.8        & 4.01E-03 & 3.53E-03 & 2.98E-03 & 3.30E-03 & 2.98E-03 & 3.01E-03 \\
        1          & 4.57E-03 & 4.11E-03 & 3.28E-03 & 3.69E-03 & 3.34E-03 & 3.35E-03 \\ \bottomrule
    \end{tabular}
\end{table}
%</tab:3drvresos>

%<*tab:3dsvresosmass>
\begin{table}[ht]
    \centering
    \caption{Mass errors in 3D single vortex test with a $32 \times 32 \times 64$ mesh, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:3drvresos} (b)}
    \label{tab:3dsvresosmass}
    \begin{tabular}{@{}lllllll@{}}
        \toprule
        CFL number & EI       & LE        & EILE3D    & EILE3DS   & EIEALE    & WY        \\ \midrule
        0.05       & 1.33E-02 & -1.33E-02 & 3.10E-13  & -1.50E-05 & 5.04E-07  & 2.98E-14  \\
        0.1        & 2.68E-02 & -2.62E-02 & 1.73E-13  & -2.50E-05 & 2.32E-06  & 1.50E-14  \\
        0.15       & 4.06E-02 & -3.86E-02 & 1.36E-13  & 3.33E-04  & 4.89E-06  & 3.56E-14  \\
        0.2        & 5.38E-02 & -5.14E-02 & 9.48E-14  & -9.60E-05 & 1.90E-06  & 2.65E-14  \\
        0.25       & 6.70E-02 & -6.35E-02 & 8.15E-14  & -1.81E-04 & 3.63E-06  & 2.15E-14  \\
        0.3        & 8.11E-02 & -7.40E-02 & 6.67E-14  & 4.59E-04  & 9.18E-06  & 2.48E-14  \\
        0.5        & 1.34E-01 & -1.19E-01 & -1.02E+01 & -8.59E-04 & -1.73E-05 & 1.63E-14  \\
        0.8        & 2.13E-01 & -1.77E-01 & -2.37E+01 & -1.84E-03 & -2.71E-04 & -5.72E-04 \\
        1          & 2.67E-01 & -2.10E-01 & -2.95E+01 & -2.69E-03 & -1.89E-04 & -3.36E-04 \\ \bottomrule
    \end{tabular}
\end{table}
%</tab:3dsvresosmass>


%<*tab:3drvresosmass>
\begin{table}[ht]
    \centering
    \caption{Mass errors in 3D reversed vortex test with a $64 \times 64 \times 64$ mesh, using different MOF advection methods. The data corresponds with the line plots in Fig. \ref{fig:3drvresos} (b)}
    \label{tab:3drvresosmass}
    \begin{tabular}{@{}lllllll@{}}
        \toprule
        CFL number & EI       & LE        & EILE3D   & EILE3DS  & EIEALE   & WY       \\ \midrule
        0.05       & 3.95E-03 & -3.95E-03 & 1.67E-13 & 3.00E-06 & 6.24E-08 & 1.41E-13 \\
        0.1        & 7.89E-03 & -7.90E-03 & 6.60E-14 & 1.30E-05 & 3.50E-07 & 7.89E-14 \\
        0.15       & 1.18E-02 & -1.19E-02 & 7.48E-14 & 2.70E-05 & 1.10E-06 & 5.84E-14 \\
        0.2        & 1.58E-02 & -1.58E-02 & 5.44E-14 & 5.40E-05 & 2.09E-06 & 4.88E-14 \\
        0.25       & 1.97E-02 & -1.98E-02 & 4.85E-14 & 8.10E-05 & 3.99E-06 & 3.47E-14 \\
        0.3        & 2.36E-02 & -2.37E-02 & 4.21E-14 & 1.08E-04 & 7.46E-06 & 2.88E-14 \\
        0.5        & 3.93E-02 & -3.95E-02 & 2.86E-14 & 3.25E-04 & 3.69E-05 & 2.26E-14 \\
        0.8        & 6.26E-02 & -6.33E-02 & 1.40E-14 & 8.46E-04 & 1.61E-04 & 1.48E-05 \\
        1          & 7.80E-02 & -7.90E-02 & 1.94E-14 & 1.33E-03 & 3.81E-04 & 1.71E-04 \\ \bottomrule
    \end{tabular}
\end{table}
%</tab:3drvresosmass>

%<*tab:comparemethods2d1>
\begin{table}[htbp]
    \centering
    \caption{Summary of 2D advection methods}
    \label{tab:comparemethods2d}
    \begin{tabular}{llllll}
        \toprule
        Method & Expression & $P_m$      & $P_g$ & $n_s$ & CFL limit \\ \midrule
        EI     &
        $\begin{aligned}
                 & C_{i,j}^{(1)} = ( C_{i,j}^{n}   + {\rm{d}}F_{i,j}^{u} ) / ( 1 - {\rm{d}}u_{i,j}) \\
                 & C_{i,j}^{n+1} = ( C_{i,j}^{(1)} + {\rm{d}}F_{i,j}^{v} ) / ( 1 - {\rm{d}}v_{i,j})
            \end{aligned}$
               & $\times$   & $\bigcirc$ & 2     & 1/2               \\ \midrule
        LE     &
        $\begin{aligned}
                 & C_{i,j}^{(1)} = ( 1 + {\rm{d}}u_{i,j})( C_{i,j}^{n}   + {\rm{d}}F_{i,j}^{u} ) \\
                 & C_{i,j}^{n+1} = ( 1 + {\rm{d}}v_{i,j})( C_{i,j}^{(1)} + {\rm{d}}F_{i,j}^{v} )
            \end{aligned}$
               & $\times$   & $\bigcirc$ & 2     & 1/2               \\ \midrule
        EILE2D &
        $\begin{aligned}
                 & C_{i,j}^{(1)} = ( C_{i,j}^{n}   + {\rm{d}}F_{i,j}^{u} ) / ( 1 - {\rm{d}}u_{i,j}) \\
                 & C_{i,j}^{n+1} = ( 1 + {\rm{d}}v_{i,j})( C_{i,j}^{(1)} + {\rm{d}}F_{i,j}^{v} )
            \end{aligned}$
               & $\bigcirc$ & $\bigcirc$ & 2     & 1/2               \\ \midrule
        LEEI2D &
        $\begin{aligned}
                 & C_{i,j}^{(1)} = ( 1 + {\rm{d}}u_{i,j})( C_{i,j}^{n}   + {\rm{d}}F_{i,j}^{u} )    \\
                 & C_{i,j}^{n+1} = ( C_{i,j}^{(1)} + {\rm{d}}F_{i,j}^{v} ) / ( 1 - {\rm{d}}v_{i,j})
            \end{aligned}$
               & $\times$   & $\bigcirc$ & 2     & 1/2               \\ \midrule
        WY     &
        $\begin{aligned}
                 & C_{i,j}^{(1)} = ( C_{i,j}^{n}   + {\rm{d}}F_{i,j}^{u} ) + \tilde{C} {\rm{d}}u_{i,j} \\
                 & C_{i,j}^{n+1} = ( C_{i,j}^{(1)} + {\rm{d}}F_{i,j}^{v} ) + \tilde{C} {\rm{d}}v_{i,j}
            \end{aligned}$
               & $\bigcirc$ & $\times$   & 2     & 1/4               \\ \midrule
    \end{tabular}
\end{table}
%</tab:comparemethods2d1>

%<*tab:comparemethods3d1>
\begin{table}[ht]
    \centering
    \caption{Summary of 3D advection methods}
    \label{tab:comparemethods3d}
    \begin{tabular}{|l|l|l|l|l|l|}
        \toprule
        Method   & Expression & $P_m$      & $P_g$ & $n_s$ & CFL limit \\ \midrule
        EI       &
        $\begin{aligned}
                 & C_{i,j}^{(1)} = ( C_{i,j}^{n}   + {\rm{d}}F_{i,j}^{u} ) / ( 1 - {\rm{d}}u_{i,j})   \\
                 & C_{i,j}^{(2)} = ( C_{i,j}^{(1)}   + {\rm{d}}F_{i,j}^{v} ) / ( 1 - {\rm{d}}v_{i,j}) \\
                 & C_{i,j}^{n+1} = ( C_{i,j}^{(2)} + {\rm{d}}F_{i,j}^{v} ) / ( 1 - {\rm{d}}w_{i,j})
            \end{aligned}$
                 & $\times$   & $\bigcirc$ & 3     & 1/2               \\ \hline
        LE       &
        $\begin{aligned}
                 & C_{i,j}^{(1)} = ( 1 + {\rm{d}}u_{i,j})( C_{i,j}^{n}   + {\rm{d}}F_{i,j}^{u} )   \\
                 & C_{i,j}^{(2)} = ( 1 + {\rm{d}}v_{i,j})( C_{i,j}^{(1)}   + {\rm{d}}F_{i,j}^{v} ) \\
                 & C_{i,j}^{n+1} = ( 1 + {\rm{d}}w_{i,j})( C_{i,j}^{(2)} + {\rm{d}}F_{i,j}^{w} )
            \end{aligned}$
                 & $\times$   & $\bigcirc$ & 3     & 1/2               \\ \hline
        EILE3D   &
        $\begin{aligned}
                 & C_{i,j}^{(1)} = ( C_{i,j}^{n}   + {\rm{d}}F_{i,j}^{\bar{u_1}} ) / ( 1 - {\rm{d}}\bar{u}_{1_{i,j}})   \\
                 & C_{i,j}^{(2)} = ( 1 + {\rm{d}}v_{1_{i,j}})( C_{i,j}^{(1)}   + {\rm{d}}F_{i,j}^{v} )                  \\
                 & C_{i,j}^{(3)} = ( C_{i,j}^{(2)}   + {\rm{d}}F_{i,j}^{\bar{w_2}} ) / ( 1 - {\rm{d}}\bar{w}_{2_{i,j}}) \\
                 & C_{i,j}^{(4)} = ( 1 + {\rm{d}}u_{2_{i,j}})( C_{i,j}^{(1)}   + {\rm{d}}F_{i,j}^{u} )                  \\
                 & C_{i,j}^{(5)} = ( C_{i,j}^{(4)}   + {\rm{d}}F_{i,j}^{\bar{v_3}} ) / ( 1 - {\rm{d}}\bar{v}_{3_{i,j}}) \\
                 & C_{i,j}^{n+1} = ( 1 + {\rm{d}}w_{3_{i,j}})( C_{i,j}^{(1)}   + {\rm{d}}F_{i,j}^{3} )                  \\
            \end{aligned}$
                 & $\bigcirc$ & $\bigcirc$ & 6     & 1/2               \\ \hline
        EILE3DS  &
        $\begin{aligned}
                 & \rm{Odd step}:                                                                           \\
                 & C_{i,j}^{(1)} = ( C_{i,j}^{n}   + {\rm{d}}F_{i,j}^{{u}} ) / ( 1 - {\rm{d}}{u}_{{i,j}})   \\
                 & C_{i,j}^{(2)} = ( 1 + {\rm{d}}v_{{i,j}})( C_{i,j}^{(1)}   + {\rm{d}}F_{i,j}^{v} )        \\
                 & C_{i,j}^{n+1} = ( C_{i,j}^{(2)}   + {\rm{d}}F_{i,j}^{{w}} ) / ( 1 - {\rm{d}}{w}_{{i,j}}) \\
                 & \rm{Even step}:                                                                          \\
                 & C_{i,j}^{(1)} = ( 1 + {\rm{d}}u_{{i,j}})( C_{i,j}^{n}   + {\rm{d}}F_{i,j}^{u} )          \\
                 & C_{i,j}^{(2)} = ( C_{i,j}^{(1)} + {\rm{d}}F_{i,j}^{{v}} ) / ( 1 - {\rm{d}}{v}_{{i,j}})   \\
                 & C_{i,j}^{n+1} = ( 1 + {\rm{d}}w_{{i,j}})( C_{i,j}^{(2)}   + {\rm{d}}F_{i,j}^{w} )        \\
            \end{aligned}$
                 & $\times$   & $\bigcirc$ & 3     & 1/2               \\ \hline
        EI-EA-LE &
        $\begin{aligned}
                 & C_{i,j}^{(1)} = ( C_{i,j}^{n}   + {\rm{d}}F_{i,j}^{{u}} ) / ( 1 - {\rm{d}}{u}_{{i,j}})                      \\
                 & C_{i,j}^{(2)} = ( 1 - {\rm{d}}w_{{i,j}})( \frac{C_{i,j}^{(1)}}{1-{\rm{d}}u_{i,j}}   + {\rm{d}}F_{i,j}^{v} ) \\
                 & C_{i,j}^{n+1} = ( C_{i,j}^{(2)}   + {\rm{d}}F_{i,j}^{{w}} ) / ( 1 - {\rm{d}}{w}_{{i,j}})                    \\
            \end{aligned}$
                 & $\times$   & $\bigcirc$ & 3     & 1/2               \\ \hline
        WY       &
        $\begin{aligned}
                 & C_{i,j}^{(1)} = ( C_{i,j}^{n}   + {\rm{d}}F_{i,j}^{u} ) + \tilde{C} {\rm{d}}u_{i,j}   \\
                 & C_{i,j}^{(2)} = ( C_{i,j}^{(1)}   + {\rm{d}}F_{i,j}^{v} ) + \tilde{C} {\rm{d}}v_{i,j} \\
                 & C_{i,j}^{n+1} = ( C_{i,j}^{(2)} + {\rm{d}}F_{i,j}^{w} ) + \tilde{C} {\rm{d}}w_{i,j}
            \end{aligned}$
                 & $\bigcirc$ & $\times$   & 3     & 1/6               \\ \bottomrule
    \end{tabular}
\end{table}


%</tab:comparemethods3d1>


